The Spectrum of Electromagnetic Jets from Kerr Black Holes and Naked Singularities in the Teukolsky Perturbation Theory

We give a new theoretical basis for examination of the presence of the Kerr black hole (KBH) or the Kerr naked singularity (KNS) in the central engine of different astrophysical objects around which astrophysical jets are typically formed: X-ray binary systems, gamma ray bursts (GRBs), active galactic nuclei (AGN), etc. Our method is based on the study of the exact solutions of the Teukolsky master equation for electromagnetic perturbations of the Kerr metric. By imposing original boundary conditions on the solutions so that they describe a collimated electromagnetic outflow, we obtain the spectra of possible {\em primary jets} of radiation, introduced here for the first time. The theoretical spectra of primary electromagnetic jets are calculated numerically. Our main result is a detailed description of the qualitative change of the behavior of primary electromagnetic jet frequencies under the transition from the KBH to the KNS, considered here as a bifurcation of the Kerr metric. We show that quite surprisingly the novel spectra describe linearly stable primary electromagnetic jets from both the KBH and the KNS. Numerical investigation of the dependence of these primary jet spectra on the rotation of the Kerr metric is presented and discussed.

==> style1.tex <==
%% Macros written by Deimantas Galcius, VTeX, Lithuania
%% Please submit bugs or your comments to deimi@vtex.lt
%%
%% The original distribution is located at:
%% http://www.e-publications.org/springer/support/
%%
%% This style file contains additional macros and is designed to use
%% with class  "aastex.cls"
%%
%% You are free to use this style file as you see fit, provided 
%% that you do not make changes to the file. 
%% If you DO make changes, you are required to rename this file.
%%
%% It may be distributed under the terms of the LaTeX Project Public
%% License, as described in lppl.txt in the base LaTeX distribution.
%% Either version 1.0 or, at your option, any later version.
%%
%% \CharacterTable
%%  {Upper-case    \A\B\C\D\E\F\G\H\I\J\K\L\M\N\O\P\Q\R\S\T\U\V\W\X\Y\Z
%%   Lower-case    \a\b\c\d\e\f\g\h\i\j\k\l\m\n\o\p\q\r\s\t\u\v\w\x\y\z
%%   Digits        \0\1\2\3\4\5\6\7\8\9
%%   Exclamation   \!     Double quote  \"     Hash (number) \#
%%   Dollar        \$     Percent       \%     Ampersand     \&
%%   Acute accent  \'     Left paren    \(     Right paren   \)
%%   Asterisk      \*     Plus          \+     Comma         \,
%%   Minus         \-     Point         \.     Solidus       \/
%%   Colon         \:     Semicolon     \;     Less than     \<
%%   Equals        \=     Greater than  \>     Question mark \?
%%   Commercial at \@     Left bracket  \[     Backslash     \\
%%   Right bracket \]     Circumflex    \^     Underscore    \_
%%   Grave accent  \`     Left brace    \{     Vertical bar  \|
%%   Right brace   \}     Tilde         \~}
%%
%%
\NeedsTeXFormat{LaTeX2e}
\def\get@CVSdate#1Id: #2,v #3 #4 #5 #6 #7${#4}%$
\def\file@version{\get@CVSdate$Id: style1.sty, deimi Exp $}
\ProvidesPackage{style1}
             [\file@version
                 ]


%\RequirePackage[T1]{fontenc}
%\RequirePackage{times}


\rightskip\z@
\@rightskip\z@
\leftskip\z@
% Dimensions
\setlength\parindent    {12\p@}
\setlength\textwidth    {495\p@}% 174mm
\setlength\textheight   {234mm} 
\setlength\columnwidth  {239\p@}% 84mm
\setlength\columnsep    {17\p@}%  6mm



\setlength\headheight{12\p@}
\setlength\headsep   {9\p@}
\setlength\topskip   {10\p@}
\setlength\footskip  {30\p@}
\setlength\maxdepth  {.5\topskip}

\setlength\topmargin       {12mm}
\advance\topmargin by-7pt

\setlength\oddsidemargin   {18mm}% gutter margin
\setlength\evensidemargin  {18mm}% outer

\if@twocolumn
 \setlength\marginparsep {10\p@}
\else
  \setlength\marginparsep{7\p@}
\fi
\setlength\marginparpush {5\p@}

% TEXT PARAMETERS
\setlength\lineskip{1\p@}
\setlength\normallineskip{1\p@}
\renewcommand\baselinestretch{}
\setlength\parskip{0\p@}

% BREAKS
\setlength\smallskipamount{6\p@ \@plus 1\p@ \@minus 1\p@}
\setlength\medskipamount  {12.5\p@ \@plus 3\p@ \@minus 3\p@}
\setlength\bigskipamount  {25\p@ \@plus 6\p@ \@minus 3\p@}

% PAGE-BREAKING PENALTIES
%\showthe\@secpenalty
\clubpenalty=10000
\widowpenalty=10000
\displaywidowpenalty=50
\predisplaypenalty=10000   % Breaking before a math display.
\pretolerance=100          % Badness tolerance for the first pass (before hyphenation)
\tolerance=800             % Badness tolerance after hyphenation
\hbadness=800              % Badness above which bad hboxes will be shown
\emergencystretch=3\p@
\hfuzz=1\p@                % do not be to critical about boxes


\def\trim@width   {210mm}
\def\trim@height  {279mm}
\def\paper@width  {210mm}
\def\paper@height {290mm}

\AtBeginDvi{\special{papersize=\trim@width, \trim@height}}
% CENTER ON PAGE
\@tempdima=\paper@width \advance\@tempdima by-\trim@width
\divide\@tempdima by2   \advance\@tempdima by-1in
\hoffset=\@tempdima

\@tempdima=\paper@height \advance\@tempdima by-\trim@height
\divide\@tempdima by2    \advance\@tempdima by-1in
\voffset=\@tempdima

% koreguojame
\advance\voffset by5mm

\renewcommand\normalsize{%
   \@setfontsize\normalsize\@xpt{12.5\p@ plus .3\p@ minus .3\p@}%
   \abovedisplayskip 10\p@ \@plus2\p@ \@minus2\p@
   \abovedisplayshortskip 6\p@ \@plus2\p@
   \belowdisplayshortskip 6\p@ \@plus2\p@
   \belowdisplayskip \abovedisplayskip}

\renewcommand\small{%
   \@setfontsize\small\@ixpt{11\p@ plus .2\p@ minus .2\p@}%
   \abovedisplayskip 7.5\p@ \@plus4\p@ \@minus1\p@
   \belowdisplayskip \abovedisplayskip
   \abovedisplayshortskip \abovedisplayskip
   \belowdisplayshortskip \abovedisplayskip}

\renewcommand\footnotesize{%
   \@setfontsize\footnotesize\@viiipt{10\p@ plus .1pt minus .1pt}%%
   \abovedisplayskip 6\p@ \@plus4\p@ \@minus1\p@
   \belowdisplayskip \abovedisplayskip
   \abovedisplayshortskip \abovedisplayskip
   \belowdisplayshortskip \abovedisplayskip}

\renewcommand\scriptsize{\@setfontsize\scriptsize\@viipt\@viiipt}

\let\footnote@size\footnotesize



% FOOTNOTES
\setlength\footnotesep   {10\p@}% 
\setlength{\skip\footins}{18\p@ \@plus 4\p@ \@minus 2\p@}
\skip\@mpfootins = \skip\footins
%
\def\footnoterule{\kern-3\p@ \hrule \@width 108\p@ \kern 2.6\p@} % the \hrule is .4pt high
\renewcommand\@makefntext[1]{\bgroup\@makefnmark\egroup\bgroup\footnotesize #1\egroup}
\def\@makefnmark{\@textsuperscript{\normalfont\@thefnmark}}%



%  sectioning
%  skiemenavimo isjungimas
%\showthe\pretolerance
%\showthe\tolerance
%\showthe\hyphenpenalty
%\showthe\exhyphenpenalty
\def\nohyphen{\pretolerance=\@M \tolerance=\@M \hyphenpenalty=\@M \exhyphenpenalty=\@M}
\def\hyphen{\pretolerance=100\tolerance=800\hyphenpenalty=50\exhyphenpenalty=50}

\renewcommand\section{\@startsection {section}{1}{\z@}%
                                   {-\bigskipamount}%
                                   {\medskipamount}%
                                   {\normalsize\bfseries\mathversion{bold}\raggedright\nohyphen}}


\renewcommand\subsection{\@startsection {subsection}{2}{\z@}%
                                   {-\medskipamount}%
                                   {\medskipamount}%
                                   {\normalsize\nohyphen\raggedright\nohyphen}}

\renewcommand\subsubsection{\@startsection{subsubsection}{3}{\z@}%
                                   {-\medskipamount}%
                                   {\medskipamount}%
                                   {\itshape\raggedright}}

\renewcommand\paragraph{\@startsection{paragraph}{4}{\z@}%
                                   {\medskipamount}%
                                   {-10pt}%
                                   {\itshape}}

\renewcommand\subparagraph{\@startsection{subparagraph}{5}{\parindent}%
                                   {0.1pt}%
                                   {-1em}%
                                   {\itshape}}


% Format for the counter:
  \def\section@numbersep{}
  \def\subsection@numbersep{}
  \def\subsubsection@numbersep{}
  \def\paragraph@numbersep{.}
  \def\subparagraph@numbersep{.}

% Format for the counter:
\def\@seccntformat#1{{\csname #1@prefix\endcsname\csname the#1\endcsname\csname#1@numbersep\endcsname\enspace}}

% misc
\overfullrule=5pt

% Abstract

% slugcomment
\long\def\slugcomment#1{\begin{flushleft}#1\par\end{flushleft}\smallskip}

% Title
\def\raggedrightmargin#1{%
  \let\\\@centercr\@rightskip #1 plus 1fil  \rightskip\@rightskip
  \leftskip\z@skip
  \parindent\z@\nohyphen}
%
\let\@@@title\relax
\def\@@@title@fmt#1{\raggedrightmargin{15mm}\vskip21\p@\bgroup\fontsize{18}{18}\bfseries\raggedright#1\par\egroup}
\def\title#1{\markright{#1}\gdef\@@@title{\@@@title@fmt{#1}}}
\def\runningtitle#1{\markright{#1}}%
\let\shorttitle\runningtitle
\let\@@@author\relax
\def\@@@author@fmt#1{\raggedrightmargin{84mm}\vskip17\p@\bgroup\normalsize\bfseries#1
\egroup%
}
\let\@@@author\relax
\def\author#1{%
\freefootnotetext[]{#1}%
\advance\n@author by\@ne
\ifnum\n@author=1
 \add@xtok@rh{#1}\else%
   \add@xtok@rh{\space\raise1.5pt\hbox{\tiny\textbullet}\space\allowbreak\hbox{#1}}%
\fi%
}
\def\@@@author{\the\rh@authors@list}
%
\newtoks\rh@authors@list
\newcount\n@author\n@author=0
\def\n@author@{0}
\def\no@harm{\let\thanks=\@gobble\let\thanksref=\@gobble\let~\space \let\\=\space \def\protect{\noexpand\protect\noexpand}}
\def\add@xtok@rh#1{\begingroup
  \no@harm  
  \def\altaffilmark##1{\textsuperscript{##1}}%
  \xdef\@act{\global\noexpand\rh@authors@list{\the\rh@authors@list#1}}\@act
\endgroup}
\def\shortauthor#1{\markboth{#1}{#1}}


%% First page 
\newdimen\@@@firstpageskip
\newdimen\@@@topboxheight
\@@@topboxheight=68mm
\@@@firstpageskip=\@@@topboxheight\relax\advance\@@@firstpageskip by-.5\baselineskip
\AtBeginDocument{\enlargethispage{-\@@@firstpageskip}}
\def\@texttop{{\thispagestyle{copyright}\twocolumn[\vtop to\@@@topboxheight{\@@@title\par\@@@author@fmt{\expandafter\@@@author}\par\@@@copyright}]}\relax\global\let\@texttop\relax}




\def\authorskip{\vskip0pt}
% Author
\def\make@author#1{% 
 {\topsep\z@\normalsize#1}% 
}% 


% Affilation
%
\def\freefootnotetext[#1]{%
       \begingroup\unrestored@protected@xdef\@thefnmark{#1}\endgroup\@footnotetext}

\def\affil{\freefootnotetext[]}

%% Abstract
\def\normaltext{\normalfont\normalsize}
\def\abstract@style{\normaltext}
\def\abstract@size{\normalsize}
\def\abstract@skip{\z@}
\def\abstractname@size{\bfseries}
\def\abstractname{Abstract}
\def\abstract{%
     \leavevmode
     \setbox\z@=\lastbox
     \abstract@style%
     \abstract@size%
     \noindent{\abstractname@size\abstractname}\enskip\ignorespaces}

\def\endabstract{\par}



%% Keywords 
\def\keyword@skip{\medskipamount}
\def\keyword@style{\normaltext\raggedright}
\def\keyword@size{\normalsize\raggedright}
\def\keyword@postfix{\unskip.}
\def\keywordname@size{\bfseries}
\def\keyword@name{Keywords}
\def\keywords#1{%
\bgroup
  \vskip\keyword@skip
%
  \keyword@style%
  \keyword@size%
  \noindent{\keywordname@size\keyword@name}\enspace#1\egroup\par}


% Footnote rule
\def\footnoterule@width{\columnwidth}
\def\footnoterule{\kern-3\p@ \hrule \@width \footnoterule@width \kern 2.6\p@} % the \hrule is .4pt high
%
\let\maketitle@runin\relax
\let\maketitle\relax
\def\altaffiltext#1#2{\freefootnotetext[#1]{#2}}

% Figure
\def\fnum@figure{{\bfseries Fig.~\thefigure\enskip}}
\def\figure@size{\small}
\let\caption@size\figure@size
\long\def\@makecaption#1#2{\bgroup\csname caption@size\endcsname\vskip
  2ex\noindent#1\ #2\par\egroup\expandafter\csname \@captype captionskip\endcsname}%
\long\def\@maketablecaption#1#2{\bgroup\csname
  caption@size\endcsname\vskip 2ex\noindent#1\
  #2\par\egroup \expandafter\csname \caption@type captionskip\endcsname}%
\def\tablecaptionskip{\vskip4pt}
\def\figurecaptionskip{\vskip0pt}

% Table 
\def\fnum@table{{\bfseries Table \thetable}\enskip}
\def\fnum@ptable@aj{{\bfseries Table \thetable}\enskip}%
\def\fnum@ptable{{\bfseries Table \thetable}\enskip}%
\def\fnum@ptablecont{{\bfseries Table \thetable}---{\rmfamily Continued}}%
\long\def\@make@caption@text#1#2{%
 \center\rmfamily#1\enskip#2\endcenter
}%


\def\@tablenotetext#1#2{%
 \vspace{.5ex}%
 {\noindent{$^{#1}$}#2\par}%
}%
\def\@tablenotes#1{%
 \par
 \vspace{4.5ex}\@gobble{\footnoterule\vspace{.5ex}}%
 {\footnotesize#1}%
}%
\def\@tablenotes@pptt#1{%
 \par
 \vspace{3.2ex}\@gobble{\footnoterule\vspace{.4ex}}%
 {\footnotesize#1}%
}%

\renewcommand\tablecomments[1]{\ifdim\@abovenoteskip=0pt\global\@abovenoteskip=10pt\fi
\appgdef\tblnote@list{\hsize\pt@width\leftskip\z@\rightskip\z@%
\@tablecom{\parfillskip\z@ plus1fil#1\endgraf}}}%
\def\@tablecom#1{%
 \par
 \vspace*{3ex}%
 {%\parbox{\pt@width} %%%
{\hskip0em\rmfamily\textit{Note}:\enskip\enskip #1}\par}%
}%
\def\@tableref@pptt#1{%
 \par
 \vspace*{3ex}%
 {%\parbox{\pt@width} %%%
 {\hskip0em{\textit{References}:\enskip\enskip #1}\par}%
}%
\def\@tablecom@pptt#1{%
 \vspace*{3ex}{%
  %\parbox{\pt@width} %%%
  {\hskip1em{\textit{Note}:\enskip\enskip #1\par}%
}%
}}
}
% Math
% flushleft
\IfFileExists{amsmath.sty}{\RequirePackage[fleqn]{amsmath}%
\setlength\mathindent\z@}%

\setlength\mathindent\z@

%% Snippet from vsfleqn2.sty
\def\mathtrivlist{\parsep\parskip\topsep\abovedisplayskip
  \ifnum\@listdepth>0 \advance\mathindent by-\leftmargin\fi%
  \@trivlist \labelwidth\z@ \leftmargin\z@
  \itemindent\z@ \def\makelabel##1{##1}}

\def\endmathtrivlist{\endtrivlist}
% \[ \]
\renewcommand\[{\relax
                \ifmmode\@badmath
                \else
                  \begin{mathtrivlist}%
                    \@beginparpenalty\predisplaypenalty
                    \@endparpenalty\postdisplaypenalty
                    \item[]\leavevmode
                    \hb@xt@\linewidth\bgroup $\m@th\displaystyle %$
                      \hskip\mathindent\bgroup
                \fi}
\renewcommand\]{\relax
                \ifmmode
                      \egroup $\hfil% $
                    \egroup
                  \end{mathtrivlist}%
                \else \@badmath
                \fi}

%%

% EQNARRAY
\renewenvironment{eqnarray}{%
    \stepcounter{equation}%
    \def\@currentlabel{\p@equation\theequation}%
    \global\@eqnswtrue\m@th
    \global\@eqcnt\z@
    \tabskip\mathindent
    \let\\=\@eqncr
%    \setlength\abovedisplayskip{\topsep}%
%    \ifvmode
%      \addtolength\abovedisplayskip{\partopsep}%
%    \fi
%    \addtolength\abovedisplayskip{\parskip}%
%    \setlength\belowdisplayskip{\abovedisplayskip}%
    \setlength\belowdisplayshortskip{\abovedisplayskip}%
    \setlength\abovedisplayshortskip{\abovedisplayskip}%
    $$\everycr{}\halign to\linewidth% $$
    \bgroup
      \hskip\@centering
      $\displaystyle\tabskip\z@skip{##}$\@eqnsel&%
      \global\@eqcnt\@ne \hskip \tw@\arraycolsep \hfil${##}$\hfil&%
      \global\@eqcnt\tw@ \hskip \tw@\arraycolsep
        $\displaystyle{##}$\hfil \tabskip\@centering&%
      \global\@eqcnt\thr@@
        \hb@xt@\z@\bgroup\hss##\egroup\tabskip\z@skip\cr}%
      {\@@eqncr
    \egroup
    \global\advance\c@equation\m@ne$$% $$
    \@ignoretrue
    }


%% Lists

\def\list@parindent{1pc}

% enumerate
\def\enumerate@indent{\z@}
\def\enumerate@parindent{\list@parindent}
\def\enumerate@labelsep{.5em}
\def\enumerate@firsttopsep{\smallskipamount}
\def\enumerate@topsep{\z@}
\def\enumerate@rightskip{\z@}% {\z@ plus 1fill}
\let\enumerate@hook\relax

% description
\def\description@indent{\list@parindent}
\let\description@topsep\smallskipamount
\let\description@hook\relax

% quotation
\let\quotation@size\footnotesize
\def\quotation@itemindent{\list@parindent}
\def\quotation@parindent{\list@parindent}
\def\quotation@leftmargin{\list@parindent}
\def\quotation@rightmargin{\z@}
\let\quotation@topsep\smallskipamount


% quote
\let\quote@size\footnotesize
\def\quote@indent{\z@}
\def\quote@leftmargin{0pc}
\def\quote@rightmargin{0pc}
\let\quote@topsep\smallskipamount



%%%%%%%%%%%%%% Parameters
\@lowpenalty   51
\@medpenalty  151
\@highpenalty 301
\@beginparpenalty -\@lowpenalty
\@endparpenalty   -\@lowpenalty
\@itempenalty     -\@lowpenalty


%%%%%%%%%%%%%% General list parameters (not important}

\parsep\z@
\topsep\z@
\partopsep\z@
\itemsep\z@
\labelsep.5em

\def\@listi  {\leftmargin\leftmargini}

\def\@listii {\leftmargin\leftmarginii%
             \labelwidth\leftmarginii%
             \advance\labelwidth-\labelsep}%

\def\@listiii{\leftmargin\leftmarginiii
              \labelwidth\leftmarginiii
              \advance\labelwidth-\labelsep}

\def\@listiv {\leftmargin\leftmarginiv
              \labelwidth\leftmarginiv
              \advance\labelwidth-\labelsep}

\def\@listvi {\leftmargin\leftmarginvi
              \labelwidth\leftmarginvi
              \advance\labelwidth-\labelsep}

\setlength\leftmargini   {2em}
\setlength\leftmarginii  {2.2em}
\setlength\leftmarginiii {1.87em}
\setlength\leftmarginiv  {1.7em}
\setlength\leftmarginv   {1em}
\setlength\leftmarginvi  {1em}

\@listi
\def\enumerate{\@ifnextchar[{\@enumerate}{\@enumerate[]}}

\def\@enumerate[#1]{%
    \ifnum \@enumdepth >\thr@@ \@toodeep\else
    \advance\@enumdepth \@ne 
    \edef\@enumctr{enum\romannumeral\the\@enumdepth}%
    \list {\csname label\@enumctr\endcsname}%
       {\usecounter{\@enumctr}
        \def\makelabel##1{{\hfill\normalfont ##1}}
%
        \ifx.#1.%
           \setcounter{\@enumctr}{3}% 
           \expandafter\settowidth\expandafter\labelwidth\expandafter{\csname label\@enumctr\endcsname}%
           \setcounter{\@enumctr}{0}%
        \else%
           \settowidth{\labelwidth}{#1}
        \fi%
        \labelsep=\enumerate@labelsep%
        \itemindent=\labelwidth \advance\itemindent\labelsep%
        \ifnum \@enumdepth=1\advance\itemindent by\enumerate@indent\fi%
        \leftmargin=\the\itemindent%
        \itemindent\z@%
        \partopsep\z@  \parsep\z@ \itemsep\z@ \rightmargin\z@
        \ifnum \@enumdepth=1 \topsep\enumerate@firsttopsep \else \topsep\enumerate@topsep\fi%
        \listparindent\enumerate@parindent%        
        \@rightskip\enumerate@rightskip%
        \enumerate@hook% 
        }\fi}

\let\endenumerate =\endlist


% itemize
\def\itemize@indent{\z@}
\def\itemize@parindent{\list@parindent}
\def\itemize@labelsep{.5em}
\def\itemize@firsttopsep{\smallskipamount}
\def\itemize@topsep{\z@}
\def\itemize@rightskip{\z@}% {\z@ plus 1fill}
\let\itemize@hook\relax

\def\labelitemi  {\textbullet}
\def\labelitemii {\textendash}
\def\labelitemiii{\textasteriskcentered} 
\def\labelitemiv {{\footnotesize +}}

\def\itemize{\@ifnextchar[{\@itemize}{\@itemize[]}}

\def\@itemize[#1]{%
    \ifnum \@itemdepth >\thr@@ \@toodeep\else
    \advance\@itemdepth \@ne 
    \edef\@itemitem{labelitem\romannumeral\the\@itemdepth}%
    \list {\csname\@itemitem\endcsname}%
       {\def\makelabel##1{{\hfill\normalfont ##1}}        
%
        \ifx.#1.%
           \settowidth\labelwidth{\csname\@itemitem\endcsname}%
        \else%
           \settowidth{\labelwidth}{#1}
        \fi%
        \labelsep=\itemize@labelsep%
        \itemindent=\labelwidth \advance\itemindent\labelsep%
        \ifnum \@itemdepth=1\advance\itemindent by\itemize@indent\fi%
        \leftmargin=\the\itemindent%
        \itemindent\z@%
        \partopsep\z@  \parsep\z@ \itemsep\z@ \rightmargin\z@
        \ifnum \@itemdepth=1 \topsep\itemize@firsttopsep \else \topsep\itemize@topsep\fi%
        \listparindent\itemize@parindent%        
        \@rightskip\itemize@rightskip%
        \itemize@hook% 
        }\fi}

\let\enditemize =\endlist


%%%%%%%%%%%%%%  description

\def\description{%
         \list{}{\labelwidth\z@ \labelsep\z@  \rightmargin\z@
         \leftmargin\z@ \advance\leftmargin by\description@indent
         \itemindent-\description@indent
         \partopsep\z@ \topsep\description@topsep \parsep\z@
         \itemsep\z@ \listparindent\z@
         \description@hook%
         \let\makelabel\descriptionlabel}}

\def\enddescription{\endlist}

\def\descriptionlabel#1{\if.#1.\else\bfseries #1\hskip.5em\fi}

%%%%%%%%%%%%%%  quotation

\def\quotation{%
        \list{}{\quotation@size%
        \listparindent\quotation@parindent%
        \itemindent   \quotation@itemindent%
        \rightmargin\quotation@rightmargin
        \leftmargin\quotation@leftmargin%
        \setlength\rightmargin{0pt}
        \partopsep\z@ \topsep\quotation@topsep \parsep\z@%
         \itemsep\z@
                        }%
        \item[\Q@strut]\relax}

\def\endquotation{\endlist}

\def\Q@strut{\leavevmode\hbox{\vrule height9pt depth1pt width0pt}}

%%%%%%%%%%%%%%  quote

\def\quote{%
        \list{}{\quote@size%
        \listparindent\quote@indent%
        \itemindent \listparindent%
        \rightmargin\quote@rightmargin   \leftmargin\quote@leftmargin%
        \partopsep\z@ \topsep\quote@topsep \parsep\z@%
                       }%
        \item\relax}

\def\endquote{\endlist}




% Acknowledgements
\def\acknowledgments{\medskip\noindent\bgroup\bfseries Acknowledgements\egroup\quad\ignorespaces}
\def\acknowledgment{\medskip\noindent\bgroup\bfseries Acknowledgement\egroup\quad\ignorespaces}

% Running head'ai
% Normalus RH
\let\headline@hook\relax
\def\rh@rule{\leavevmode\lower6pt\hbox to0pt{\vrule height1pt width\textwidth\hss}}
\def\rh@rule@{\leavevmode\lower18pt\hbox to0pt{\vrule height1pt width\textwidth\hss}}
\def\thepage@fmt#1{#1}
\def\runninghead@size {\footnotesize}
\def\pagenumber@size {\footnotesize}
\def\ps@headings{%
      \def\@evenfoot{\@empty}%
      \def\@oddfoot{\@empty}%
      \def\@evenhead{\headline@hook\rh@rule\runninghead@size\rlap{\pagenumber@size\thepage@fmt{\thepage}}\hfill\leftmark}%
      \def\@oddhead{\headline@hook\rh@rule\runninghead@size\rightmark\hfill\llap{\pagenumber@size\thepage@fmt{\thepage}}}%
}
% Copyright RH
\def\cp@text{\parbox[t]{\textwidth}}
\def\ps@copyright{%
      \def\@evenfoot{\@empty}%
      \def\@oddfoot{\@empty}%
      \def\@evenhead{\headline@hook\rh@rule@\runninghead@size\rlap{\pagenumber@size\thepage@fmt{\@gobble\thepage}}\hfill\leftmark}%
      \def\@oddhead{\headline@hook\rh@rule@\runninghead@size\hfill\cp@text\llap{\pagenumber@size\thepage@fmt{\@gobble\thepage}}}%
}

\pagestyle{headings}
% % pirmas puslapis
\def\@jname{}
\def\@doi{\@doihead \@thedoi}
\def\@doihead{DOI:\space}
\def\@thedoi{10.1007/\textbullet\textbullet\textbullet\textbullet\textbullet-\textbullet\textbullet\textbullet-\textbullet\textbullet\textbullet-\textbullet\textbullet\textbullet\textbullet-\textbullet}
%

% References
\def\refname{References}
\renewenvironment{thebibliography}[1]{% 
 \clear@thebibliography@page 
 \section*{\refname}% 
 \thebib@list 
 \def\refpar{\relax}% 
 \def\newblock{\hskip .11em\@plus.33em\@minus.07em}% 
 \clubpenalty4000 
 \widowpenalty4000 
 \sfcode`\.=1000\relax 
}{% 
 \endlist 
 \revtex@pageid 
}% 

\def\thebib@list{% 
 \list{\null}{% 
   \small
  \leftmargin 1em\labelwidth\z@\labelsep\z@\itemindent-\leftmargin 
 \global\setlength\bibsep\z@ 
 \global\itemsep=\z@ \@plus1\p@ \@minus1\p@
 \global\parsep=\z@ \@plus1\p@ \@minus1\p@
  \usecounter{enumi}% 
 }% 
}% 


\def\@coprtyear{\textbullet\textbullet\textbullet\textbullet} 
\def\@volume{0}
\def\@@firstpage{\textbullet}
\def\@@lastpage{\textbullet}
\def\mymyleftmark{\@jname\@gobble{\ (\@coprtyear) \@volume:\@firstpage--\@lastpage}}


% Twoside printing
\@twosidetrue\@mparswitchtrue
\twocolumn

% Redefining Journal Acronyms
\renewcommand\aj{\ref@jnl{Astron.~J.}}%
          % Astronomical Journal
\renewcommand\actaa{\ref@jnl{Acta Astron.}}%
          % Acta Astronomica
\renewcommand\araa{\ref@jnl{Annu. Rev. Astron. Astrophys.}}%
          % Annual Review of Astron and Astrophys
\renewcommand\apj{\ref@jnl{Astrophys.~J.}}%
          % Astrophysical Journal
\renewcommand\apjl{\ref@jnl{Astrophys. J. Lett.}}%
          % Astrophysical Journal, Letters
\renewcommand\apjs{\ref@jnl{Astrophys. J. Suppl. Ser.}}%
          % Astrophysical Journal, Supplement
\renewcommand\ao{\ref@jnl{Appl. Opt.}}%
          % Applied Optics
\renewcommand\apss{\ref@jnl{Astrophys. Space Sci.}}%
          % Astrophysics and Space Science
\renewcommand\aap{\ref@jnl{Astron. Astrophys.}}%
          % Astronomy and Astrophysics
\renewcommand\aapr{\ref@jnl{Astron. Astrophys. Rev.}}%
          % Astronomy and Astrophysics Reviews
\renewcommand\aaps{\ref@jnl{Astron. Astrophys. Suppl. Ser.}}%
          % Astronomy and Astrophysics, Supplement
\renewcommand\azh{\ref@jnl{Astron. Zh.}}%
          % Astronomicheskii Zhurnal
\renewcommand\baas{\ref@jnl{Bull. Am. Astron. Soc.}}%
          % Bulletin of the AAS
\renewcommand\caa{\ref@jnl{Chin. Astron. Astrophys.}}%
  % Chinese Astronomy and Astrophysics
\renewcommand\cjaa{\ref@jnl{Chin. J. Astron. Astrophys.}}%
  % Chinese Journal of Astronomy and Astrophysics
\renewcommand\icarus{\ref@jnl{Icarus}}%
  % Icarus
\renewcommand\jcap{\ref@jnl{J. Cosmol. Astropart. Phys.}}%
  % Journal of Cosmology and Astroparticle Physics
\renewcommand\jrasc{\ref@jnl{J.~R. Astron. Soc. Can.}}%
          % Journal of the RAS of Canada
\renewcommand\memras{\ref@jnl{Mem. R. Astron. Soc.}}%
          % Memoirs of the RAS
\renewcommand\mnras{\ref@jnl{Mon. Not. R. Astron. Soc.}}%
          % Monthly Notices of the RAS
\renewcommand\na{\ref@jnl{New Astron.}}%
  % New Astronomy
\renewcommand\nar{\ref@jnl{New Astron. Rev.}}%
  % New Astronomy Review
\renewcommand\pra{\ref@jnl{Phys. Rev.~A}}%
          % Physical Review A: General Physics
\renewcommand\prb{\ref@jnl{Phys. Rev.~B}}%
          % Physical Review B: Solid State
\renewcommand\prc{\ref@jnl{Phys. Rev.~C}}%
          % Physical Review C
\renewcommand\prd{\ref@jnl{Phys. Rev.~D}}%
          % Physical Review D
\renewcommand\pre{\ref@jnl{Phys. Rev.~E}}%
          % Physical Review E
\renewcommand\prl{\ref@jnl{Phys. Rev. Lett.}}%
          % Physical Review Letters
\renewcommand\pasa{\ref@jnl{Proc. Astron. Soc. Aust.}}%
  % Publications of the Astron. Soc. of Australia
\renewcommand\pasp{\ref@jnl{Publ. Astron. Soc. Pac.}}%
          % Publications of the ASP
\renewcommand\pasj{\ref@jnl{Publ. Astron. Soc. Jpn.}}%
          % Publications of the ASJ
\renewcommand\qjras{\ref@jnl{Q. J. R. Astron. Soc.}}%
          % Quarterly Journal of the RAS
\renewcommand\rmxaa{\ref@jnl{Rev. Mexicana Astron. Astrofis.}}%
  % Revista Mexicana de Astronomia y Astrofisica
\renewcommand\skytel{\ref@jnl{Sky Telesc.}}%
          % Sky and Telescope
\renewcommand\solphys{\ref@jnl{Sol. Phys.}}%
          % Solar Physics
\renewcommand\sovast{\ref@jnl{Soviet Astron.}}%
          % Soviet Astronomy
\renewcommand\ssr{\ref@jnl{Space Sci. Rev.}}%
          % Space Science Reviews
\renewcommand\zap{\ref@jnl{Z. Astrophys.}}%
          % Zeitschrift fuer Astrophysik
\renewcommand\nat{\ref@jnl{Nature}}%
          % Nature
\renewcommand\iaucirc{\ref@jnl{IAU Circ.}}%
          % IAU Cirulars
\renewcommand\aplett{\ref@jnl{Astrophys. Lett.}}%
          % Astrophysics Letters and Communications
\renewcommand\apspr{\ref@jnl{Astrophys. Space Phys. Res.}}%
          % Astrophysics Space Physics Research
\renewcommand\bain{\ref@jnl{Bull. Astron. Inst. Neth.}}%
          % Bulletin Astronomical Institute of the Netherlands
\renewcommand\fcp{\ref@jnl{Fundam. Cosmic Phys.}}%
          % Fundamental Cosmic Physics
\renewcommand\gca{\ref@jnl{Geochim. Cosmochim. Acta}}%
          % Geochimica Cosmochimica Acta
\renewcommand\grl{\ref@jnl{Geophys. Res. Lett.}}%
          % Geophysics Research Letters
\renewcommand\jcp{\ref@jnl{J. Chem. Phys.}}%
          % Journal of Chemical Physics
\renewcommand\jgr{\ref@jnl{J. Geophys. Res.}}%
          % Journal of Geophysical Research
\renewcommand\jqsrt{\ref@jnl{J. Quant. Spec. Radiat. Transf.}}%
          % Journal of Quantitiative Spectroscopy and Radiative Trasfer
\renewcommand\memsai{\ref@jnl{Mem. Soc. Astron. Italiana}}%
          % Mem. Societa Astronomica Italiana
\renewcommand\nphysa{\ref@jnl{Nucl. Phys.~A}}%
          % Nuclear Physics A
\renewcommand\physrep{\ref@jnl{Phys. Rep.}}%
          % Physics Reports
\renewcommand\physscr{\ref@jnl{Phys. Scr.}}%
          % Physica Scripta
\renewcommand\planss{\ref@jnl{Planet. Space Sci.}}%
          % Planetary Space Science
\renewcommand\procspie{\ref@jnl{Proc. SPIE}}%
          % Proceedings of the SPIE
\let\astap=\aap
\let\apjlett=\apjl
\let\apjsupp=\apjs
\let\applopt=\ao

%% vtexfix
\DeclareFontShape{OMS}{cmsy}{b}{n}{%
      <-6> cmbsy5 <6-8> cmbsy7 <8-> cmbsy10%
      }{}


\endinput

